Reducing Communication in Graph Neural Network Training

Graph Neural Networks (GNNs) are powerful and flexible neural networks that use the naturally sparse connectivity information of the data. GNNs represent this connectivity as sparse matrices, which have lower arithmetic intensity and thus higher communication costs compared to dense matrices, making GNNs harder to scale to high concurrencies than convolutional or fully-connected neural networks. We introduce a family of parallel algorithms for training GNNs and show that they can asymptotically reduce communication compared to previous parallel GNN training methods. We implement these algorithms, which are based on 1D, 1.5D, 2D, and 3D sparse-dense matrix multiplication, using torch.distributed on GPU-equipped clusters. Our algorithms optimize communication across the full GNN training pipeline. We train GNNs on over a hundred GPUs on multiple datasets, including a protein network with over a billion edges.

==> partscheme1_old.tex <==
% \subsection{Partitioning Scheme 1}
% \subsubsection{Partitioning Description}
% \begin{table}[!h]
% \centering
% \begin{tabular}{ |p{2cm}||p{3cm}|}
% \hline
% Matrix & Partitioning  \\
% \hline
% $A$ & Column-based\\
% $H^l$ & Fully-replicated \\
% $G^l$ & Fully-replicated \\
% $W^l$ & Fully-replicated\\
% \hline 
% \end{tabular}
% \end{table}
% \subsubsection{Equation $H^l = A^TH^{l - 1}W^l$}
% \begin{figure}[h]
%     \centering
%     \includegraphics[scale=0.4]{ps1eq1.png}
%     \caption{Partitioning Scheme $1$ Equation $1$}
%     \label{fig:ps1eq1}
% \end{figure}
% 
% \begin{center}
%     Communication: AllGather across partitions of $H^l$
%     \begin{align*}
%         T_{comm} = \sum_{l = 1}^{L}(\alpha\log P + \beta nf\frac{P - 1}{P})
%     \end{align*}
% \end{center}
% 
% \pagebreak
% 
% \subsubsection{Equation $G^l = AG^{l + 1}W^l$}
% \begin{figure}[h]
%     \centering
%     \includegraphics[scale=0.4]{ps1eq2.png}
%     \caption{Partitioning Scheme $1$ Equation $2$}
%     \label{fig:ps1eq2}
% \end{figure}
% 
% \begin{center}
%     Communication: AllGather across partitions of $G^l$
%     \begin{align*}
%         T_{comm} = \sum_{l = 1}^{L}(\alpha\log P + \beta nf\frac{P - 1}{P})
%     \end{align*}
% \end{center}
% 
% \subsubsection{Equation $\frac{\partial \mathcal{L}}{\partial W} = (H^{l - 1})^TAG^l$}
% \begin{figure}[h]
%     \centering
%     \includegraphics[scale=0.4]{ps1eq3.png}
%     \caption{Partitioning Scheme $1$ Equation $3$}
%     \label{fig:ps1eq3}
% \end{figure}
% 
% \begin{center}
%     Communication: AllReduce across low-rank results of $\frac{\partial \mathcal{L}}{\partial W}$
%     \begin{align*}
%         T_{comm} = \sum_{l = 1}^{L}(\alpha\log P + \beta nf\frac{P - 1}{P})
%     \end{align*}
% \end{center}
% 
% \pagebreak
% 
% \subsection{Partitioning Scheme 2}
% \subsubsection{Partitioning Description}
% \begin{table}[!h]
% \centering
% \begin{tabular}{ |p{2cm}||p{3cm}|}
% \hline
% Matrix & Partitioning  \\
% \hline
% $A$ & Row-based\\
% $H^l$ & Row-based \\
% $G^l$ & Row-based \\
% $W^l$ & Fully-replicated\\
% \hline 
% \end{tabular}
% \end{table}
% \subsubsection{Equation $H^l = A^TH^{l - 1}W^l$}
% \begin{figure}[h]
%     \centering
%     \includegraphics[scale=0.4]{ps2eq1.png}
%     \caption{Partitioning Scheme $2$ Equation $1$}
%     \label{fig:ps2eq1}
% \end{figure}
% 
% \begin{center}
%     Communication: AllGather across partitions of $H^l$
%     \begin{align*}
%         T_{comm} = \sum_{l = 1}^{L}(\alpha\log P + \beta nf\frac{P - 1}{P})
%     \end{align*}
% \end{center}
% 
% \subsubsection{Equation $G^l = AG^{l + 1}W^l$}
% \begin{figure}[h]
%     \centering
%     \includegraphics[scale=0.4]{ps2eq2.png}
%     \caption{Partitioning Scheme $2$ Equation $2$}
%     \label{fig:ps2hq2}
% \end{figure}
% 
% \begin{center}
%     Communication: AllGather from multiplying two different partitions in $AG^{l + 1}$
%     \begin{align*}
%         T_{comm} = \sum_{l = 1}^{L}(\alpha\log P + \beta edgecut(A)f\frac{P - 1}{P})
%     \end{align*}
% \end{center}
% 
% \subsubsection{Equation $\frac{\partial \mathcal{L}}{\partial W} = (H^{l - 1})^TAG^l$}
% \begin{figure}[h]
%     \centering
%     \includegraphics[scale=0.4]{ps2eq3.png}
%     \caption{Partitioning Scheme $2$ Equation $3$}
%     \label{fig:ps2eq3}
% \end{figure}
% 
% \begin{center}
%     Communication: AllReduce across low-rank results of $\frac{\partial \mathcal{L}}{\partial W}$
%     \begin{align*}
%         T_{comm} = \sum_{l = 1}^{L}(\alpha\log P + \beta nf\frac{P - 1}{P})
%     \end{align*}
% \end{center}


==> partscheme2.tex <==


\subsection{Partitioning Scheme 2}
\subsubsection{Partitioning Description}
\begin{table}[!h]
\centering
\begin{tabular}{ |p{2cm}||p{3cm}|}
\hline
Matrix & Partitioning  \\
\hline
$A$ & Row-based\\
$H^l$ & Row-based \\
$G^l$ & Row-based \\
$W^l$ & Fully-replicated \\
\hline
\end{tabular}
\end{table}

\subsubsection{Equation $Z^l = A^TH^{l - 1}W^l$}
\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{ps2eq1_new.png}
    \caption{Partitioning Scheme $2$ Equation $1$}
    \label{fig:ps2eq1}
\end{figure}
\paragraph{Communication: 1D Outer Product} 
    $A^T$ is partitioned by columns, and $H^{l - 1}$ is partitioned by rows. This yields a $1$D Outer Product multiplication with an all-reduce on matrices of size $n \times f$. $W^l$ is fully-replicated on each process, and is multiplied with $A^TH^{l - 1}$ after communication.
    \begin{align*}
        W &= O(edgecut_P(A) * f) \\
        S &= O(\log P) 
    \end{align*}

\pagebreak

\subsubsection{Equation $H^l = \sigma(Z^l)$}
\paragraph{Communication: None} 
    $H^l$, the result of activation, is partitioned by rows as is $H^{l - 1}$. No further communication is necessary here to use $H^l$ in Eq. 1 for layer $l$.
    
\subsubsection{Equation $G^l = AG^{l + 1}(W^{l + 1})^T \odot \sigma '(Z^l)$}
\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{ps2eq2_new.png}
    \caption{Partitioning Scheme $2$ Equation $2$}
    \label{fig:ps2eq2}
\end{figure}
\paragraph{Communication: 1D Block Row} 
    $A$ is partitioned by rows, and $G^{l + 1}$ is partitioned by rows. This yields a $1$D Block Row multiplication. $(W^{l + 1})^T$ is fully-replicated on each process, and is multiplied with $AG^{l + 1}$ after communication.
    \begin{align*}
        W &= O(edgecut_P(A) * f) \\
        S &= O(P) 
    \end{align*}

\pagebreak

\subsubsection{Equation $\frac{\partial \mathcal{L}}{\partial W} = (H^{l - 1})^TAG^l$}
\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{ps2eq3_new.png}
    \caption{Partitioning Scheme $2$ Equation $3$}
    \label{fig:ps2eq3}
\end{figure}
\paragraph{Communication: 1D Block Row + 1D Outer Product} 
    There are two matrix multiplications here. The first is multiplying $A$ and $G^l$, which is one 1D Block Row since both $A$ and $G^l$ are partitioned by rows. The second is multiplying $(H^{l - 1})^T$ with the result of the first multiplication. This is a 1D Outer Product with an all-reduce on matrices of size $f \times f$.
    \begin{align*}
        W_1 &= O(edgecut_P(A) * f) \\
        S_1 &= O(P)  \\
        \\
        W_2 &= O(f^2) \\
        S_2 &= O(\log P) 
    \end{align*}
    
\subsubsection{Total Communication}
\begin{align*}
    T_{comm} = \sum_{l = 1}^{L}(\alpha(2\log P + 2P) + \beta(3edgecut_P(A) * f + f^2))
\end{align*}

\pagebreak



==> partscheme3.tex <==

\subsection{Partitioning Scheme 3}
\subsubsection{Partitioning Description}
\begin{table}[!h]
\centering
\begin{tabular}{ |p{2cm}||p{3cm}|}
\hline
Matrix & Partitioning  \\
\hline
$A$ & Mixed*\\
$H^l$ & Row-based \\
$G^l$ & Row-based \\
$W^l$ & Fully-replicated \\
\hline
\end{tabular}
\end{table}

*Here we transpose $A$ between forward propagation and backward propagation. This way, both $A$ and $A^T$ will be partitioned by columns when they are used. We only transpose $A$ twice per epoch (after forward propagation and after backward propagation), not once per layer.

\subsubsection{Equation $Z^l = A^TH^{l - 1}W^l$}
\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{ps2eq1_new.png}
    \caption{Partitioning Scheme $3$ Equation $1$}
    \label{fig:ps3eq1}
\end{figure}
\paragraph{Communication: 1D Outer Product} 
    $A^T$ is partitioned by columns, and $H^{l - 1}$ is partitioned by rows. This yields a $1$D Outer Product multiplication with an all-reduce on matrices of size $n \times f$. $W^l$ is fully-replicated on each process, and is multiplied with $A^TH^{l - 1}$ after communication.
    \begin{align*}
        W &= O(edgecut_P(A) * f) \\
        S &= O(\log P) 
    \end{align*}

\pagebreak

\subsubsection{Equation $H^l = \sigma(Z^l)$}
\paragraph{Communication: None} 
    $H^l$, the result of activation, is partitioned by rows as is $H^{l - 1}$. No further communication is necessary here to use $H^l$ in Eq. 1 for layer $l$.
    
\subsubsection{Transposing $A$}
\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{transA.png}
    \caption{Transposing $A$}
    \label{fig:transA}
\end{figure}
\paragraph{Communication: AllGather}
    We can run an all-gather on all $P$ processes to transpose $A$. \Aydin{Is it really Allgather (also known as concatenation~\cite{bruck1997efficient} - by the way, this paper by Bruck et al.\, that I just referenced is old but highly recommended - ) that you are looking for here? It seems like what you want is really an MPI\_Alltoallv, also known as personalized all-to-all. In fact, all-to-all used to be synonymous with ``transpose''~\cite{bader1996practical}. A rather complete (modulo Alltoallv) description of commonly used collectives in distributed memory, together with their de-facto names  can be found in the Chan et al.\, paper~\cite{chan2007collective}}
    \Alok{Yeah, I see what you mean. It's really an all-to-all, where each process splits its $\mA_i$ partition into $P$ chunks, and sends each chunk to a different processor. Would the communication complexity then be what I have in blue below now?}
    \begin{align*}
        W &= O(edgecut_P(A)) \\
        S &= O(\log P) \\
        &\Alok{W = O(dn / P)} \\
        &\Alok{S = O(P^2)} \\
    \end{align*}

\pagebreak

\subsubsection{Equation $G^l = AG^{l + 1}(W^{l + 1})^T \odot \sigma '(Z^l)$}
\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{ps1eq2_new.png}
    \caption{Partitioning Scheme $3$ Equation $2$}
    \label{fig:ps3eq2}
\end{figure}
\paragraph{Communication: 1D Outer Product} 
    $A$ is partitioned by columns, and $G^{l + 1}$ is partitioned by rows. This yields a $1$D Outer Product multiplication with an all-reduce on matrices of size $n\times f$. $(W^{l + 1})^T$ is fully-replicated on each process, and is multiplied with $AG^{l + 1}$ after communication.
    \begin{align*}
        W &= O(edgecut_P(A) * f) \\
        S &= O(\log P) 
    \end{align*}

\subsubsection{Equation $\frac{\partial \mathcal{L}}{\partial W} = (H^{l - 1})^TAG^l$}
\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{ps1eq3_new.png}
    \caption{Partitioning Scheme $3$ Equation $3$}
    \label{fig:ps2eq3}
\end{figure}
\paragraph{Communication: 2 * 1D Outer Product} 
    There are two matrix multiplications here. The first is multiplying $A$ and $G^l$, which is one 1D Outer Product with an all-reduce on matrices of size $n \times f$. The second is multiplying $(H^{l - 1})^T$ with the result of the first multiplication. This is a 1D Outer Product with an all-reduce on matrices of size $f \times f$.
    \begin{align*}
        W_1 &= O(edgecut_P(A) * f) \\
        S_1 &= O(P)  \\
        \\
        W_2 &= O(f^2) \\
        S_2 &= O(\log P) 
    \end{align*}
    
\subsubsection{Total Communication}
\begin{align*}
    T_{comm} = \sum_{l = 1}^{L}(\alpha(4\log P) + \beta(3edgecut_P(A) * f + f^2)) + 2(\alpha\log P + \beta edgecut_P(A))
\end{align*}


